Towards Score Following in Sheet Music Images

This paper addresses the matching of short music audio snippets to the corresponding pixel location in images of sheet music. A system is presented that simultaneously learns to read notes, listens to music and matches the currently played music to its corresponding notes in the sheet. It consists of an end-to-end multi-modal convolutional neural network that takes as input images of sheet music and spectrograms of the respective audio snippets. It learns to predict, for a given unseen audio snippet (covering approximately one bar of music), the corresponding position in the respective score line. Our results suggest that with the use of (deep) neural networks -- which have proven to be powerful image processing models -- working with sheet music becomes feasible and a promising future research direction.

==> reviews <==
Dear Mr. Matthias Dorfer,

Congratulations! We would like to inform you that your paper

      Towards Reading Sheet Music (Paper #27)

has been scheduled for ORAL presentation at ISMIR 2016. (Please note that all ORAL and POSTER contributions are considered to have the same status at ISMIR.)

In this email you will find the following information:
 1) Camera-Ready Submission Instructions
 2) Author Registration Deadline
 3) Registration and Accommodation Information
 4) Financial Support (ThinkTank, Women in Music IR & Students Grants)
 5) Reviews for your Paper  

All the best,

Johanna Devaney
Douglas Turnbull
George Tzanetakis
Program Chairs, ISMIR 2016

Juan Bello
Dan Ellis
General Chairs, ISMIR 2016


===== 1) Camera Ready Submission =====

Your next step is to prepare a camera-ready manuscript by:

     *** Camera-Ready Deadline: Friday, May 27 ***

You should de-anonymize your papers, add acknowledgements when appropriate, and make updates based on the feedback from the reviewers (see below). When revising your papers, make sure that all fonts are embedded in the PDF document, and that it is not password-protected. Papers which are not formatted according to the ISMIR 16 templates (including excessive use of \baselinestretch) or papers that exceed the 6+1 page length requirement will not be accepted for publication in the proceedings.  

To submit your camera-ready manuscript, you can click on the following URL which will take you directly to a form to submit your final paper:

     https://www.softconf.com/h/ismir2016/cgi-bin/scmd.cgi?scmd=aLogin&passcode=27X-C3C7A6D2H7

We will notify you about the specific day and time of your presentation at a later date. 

===== 2) Author Registration  =====

Accepted papers must be presented at the conference by one of the authors and at least one of the authors must register by the Author Registration deadline:

   ***  Author Registration Deadline: Friday, June 3rd *** 

Failure to register before the deadline will result in automatic withdrawal of your paper from the conference proceedings and program.  

===== 3) Registration and Accommodation Information =====

We’re happy to announce that registration for the 17th Conference of the International Society for Music Information Retrieval (ISMIR-16) is now officially open. The conference will be held in New York City between August 7th and 11th, 2016, primarily at the campus of New York University (NYU).

****************
Registration:

To register for the conference and tutorials and to book discount accommodation at NYU, please visit: 
https://wp.nyu.edu/ismir2016/participants-2/registration/

The deadline for early registration and author registration is June 3. Prices will increase after this date and any papers for which there is not appropriate author registration by this date (see details in Section 2 above) will not be included in the conference or the proceedings.

Visit our site for information on tutorials, an outline of the conference program, and information on satellite events (ThinkTank, HAMR, CogMIR and DLfM).

****************
Accommodation and other travel arrangements:

Please note that NYU housing availability is limited and will be awarded on a first-come-first-served basis. Housing is restricted to people 18 years old and above, and is not suitable for families with children, or unregistered partners. Booking must be completed as part of the registration process. 

For more information about accommodation including options outside NYU, please visit:
https://wp.nyu.edu/ismir2016/participants-2/accommodation/

To help you in planning your trip, we have also prepared pages with information about visas and travel to/from NYC’s airports.


===== 4) Financial Support (Grants) =====

ISMIR and the Women in MIR (WiMIR) initiative are proud to announce a number of financial support opportunities for students and other members of the community wishing to attend the conference. Awards are granted based on the quality of the accepted submission, the degree of financial need, the applicant’s newness to ISMIR, and the applicant’s geographical diversity.

The types of awards are
ThinkTank registration - available for all grad students who are attending ISMIR.
Student Author Grants - available for first or supporting authors of an accepted full paper who were students at the time of paper submission.
Women in MIR (WiMIR) Grants - available to female first or supporting authors of accepted full papers, as well as female first authors of accepted late-breaking demo (LBD) submissions. WiMIR Grants are being offered for the first time thanks to the generous support of industry partners (Smule, Shazam). Applicants do NOT need to be students to apply for the WiMIR Award.

Details on how to apply are available at:
https://wp.nyu.edu/ismir2016/participants-2/financial-support-grants/


===== 5) Reviews for your Paper  =====

============================================================================ 
ISMIR 2016 Reviews for Submission #27
============================================================================ 

Title: Towards Reading Sheet Music

Authors: Matthias Dorfer, Andreas Arzt and Gerhard Widmer
============================================================================
                            REVIEWER #1
============================================================================ 


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

            Scholarly/scientific quality: high
                                 Novelty: high
                      Relevance of topic: high
                              Importance: medium high
      Readability and paper organisation: high
                      Title and abstract: yes
                            Bibliography: yes


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

I have liked the paper. It's an interesting idea. The criticism I have it is
alson mentioned but the authors: it only works with monophonic music.
Though, this is a paper for a conference where new ideas should be presented.
So, I think it is well suited for that.
When they extend their system to polyphonic music, they  should send it to a
journal.

============================================================================
                            REVIEWER #2
============================================================================ 


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

            Scholarly/scientific quality: medium high
                                 Novelty: medium high
                      Relevance of topic: high
                              Importance: medium high
      Readability and paper organisation: medium high
                      Title and abstract: yes
                            Bibliography: yes


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

It may be interesting to include explicitly the size of the overlapping of 
frames.

I think that the example of horizontal quantization of the sheet image into
non-overlapping buckets of Figure 2 is misleading. It seems that a note may be
cut in the middle, which is not the case, as explained later.

In the last sentence of section 3.5, where it says Fig 2, it should say Table
2, I guess.

============================================================================
                            REVIEWER #3
============================================================================ 


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

            Scholarly/scientific quality: medium low
                                 Novelty: medium low
                      Relevance of topic: high
                              Importance: medium high
      Readability and paper organisation: medium low
                      Title and abstract: no
                            Bibliography: yes


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

The topic of the paper is essentially an approach to audio to score alignment.
For this reason, I marked the title as not appropriate since the audio
component is missing and the title is misleading. 

The proposed method is at a _very_ early stage. Basically, the idea is not to
perform the alignment with symbolic data but instead to work directly with the
image. In other words, to short cut the symbolic data acquisition, or the OMR
process.

The data used is very simple, with single staves of monophonic music. This is
one the major problems with this paper. If the results, as exposed, look
promising, it is very unclear how the method can be applied to reasonably more
complex scores (or "real music" as mentioned by the authors). The method
performs some sort of built-in OMR process that it will be extremely difficult
to apply to full scores. For example, where will the segmentation will be done?
So the paper is mostly a machine learning one with not much music insights.

Also, there is no comparison with other approaches. It would have been trivial
to run an OMR on the data set an compare the results.

============================================================================
                            REVIEWER #4
============================================================================ 


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------

            Scholarly/scientific quality: medium low
                                 Novelty: high
                      Relevance of topic: medium high
                              Importance: medium high
      Readability and paper organisation: medium high
                      Title and abstract: no
                            Bibliography: yes


---------------------------------------------------------------------------
Comments
---------------------------------------------------------------------------

This is a summary review written by the PC member supervising the paper.

The title of this paper is inappropriate. Please change to something like "A
new method for audio to score alignment with monophonic music”.

As noted elsewhere, there is no comparison to existing score following methods.
Please explain why this was not done and perhaps speculate on how it would
compare.

